Practical offloading for fine-tuning LLM on commodity GPU via learned sparse projectors

Fine-tuning large language models (LLMs) requires significant memory, often exceeding the capacity of a single GPU. A common solution to this memory challenge is offloading compute and data from the GPU to the CPU. However, this approach is hampered by the limited bandwidth of commodity hardware, which constrains communication between the CPU and GPU, and by slower matrix multiplications on the CPU. In this paper, we present an offloading framework, LSP-Offload, that enables near-native speed LLM fine-tuning on commodity hardware through learned sparse projectors. Our data-driven approach involves learning efficient sparse compressors that minimize communication with minimal precision loss. Additionally, we introduce a novel layer-wise communication schedule to maximize parallelism between communication and computation. As a result, our framework can fine-tune a 1.3 billion parameter model on a 4GB laptop GPU and a 6.7 billion parameter model on a 24GB NVIDIA RTX 4090 GPU. Compared to state-of-the-art offloading frameworks, our approach reduces end-to-end fine-tuning time by 33.1%-62.5% when converging to the same accuracy. We open source our framework at https://github.com/gulang2019/LSP-Offload.

==> checklist.tex <==
\section{Checklist}
This paper:

Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)
Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)
Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no)
Does this paper make theoretical contributions? (yes/no)

If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. yes.
    \item All novel claims are stated formally (e.g., in theorem statements). yes.
    \item Proofs of all novel claims are included. yes.
    \item Proof sketches or intuitions are given for complex and/or novel results. yes.
    \item Appropriate citations to theoretical tools used are given. yes.
    \item All theoretical claims are demonstrated empirically to hold. yes.
    \item All experimental code used to eliminate or disprove claims is included. yes.
\end{itemize}

Does this paper rely on one or more datasets? yes.

If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets. yes.
    \item All novel datasets introduced in this paper are included in a data appendix. NA.
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. NA.
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. yes.
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. yes. 
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. NA.
\end{itemize}
% A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)
% All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)
% All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)
% All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)
% % All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)
% All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)
Does this paper include computational experiments? yes.

If yes, please complete the list below.

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. yes.
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. yes.
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. yes.
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. yes
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. yes.
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. yes.
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. yes.
    \item This paper states the number of algorithm runs used to compute each reported result. yes.
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. yes.
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). no.
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. yes.
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. yes.
\end{itemize}

% Any code required for pre-processing data is included in the appendix. (yes/partial/no).
% All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)
% All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)
% All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)
% If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)
% This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)
% This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)
% This paper states the number of algorithm runs used to compute each reported result. (yes/no)
% Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)
% The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)
% This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)
% This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)
